Hippocrates: An Open-Source Framework for Advancing Large Language Models in Healthcare

The integration of Large Language Models (LLMs) into healthcare promises to transform medical diagnostics, research, and patient care. Yet, the progression of medical LLMs faces obstacles such as complex training requirements, rigorous evaluation demands, and the dominance of proprietary models that restrict academic exploration. Transparent, comprehensive access to LLM resources is essential for advancing the field, fostering reproducibility, and encouraging innovation in healthcare AI. We present Hippocrates, an open-source LLM framework specifically developed for the medical domain. In stark contrast to previous efforts, it offers unrestricted access to its training datasets, codebase, checkpoints, and evaluation protocols. This open approach is designed to stimulate collaborative research, allowing the community to build upon, refine, and rigorously evaluate medical LLMs within a transparent ecosystem. Also, we introduce Hippo, a family of 7B models tailored for the medical domain, fine-tuned from Mistral and LLaMA2 through continual pre-training, instruction tuning, and reinforcement learning from human and AI feedback. Our models outperform existing open medical LLMs models by a large-margin, even surpassing models with 70B parameters. Through Hippocrates, we aspire to unlock the full potential of LLMs not just to advance medical knowledge and patient care but also to democratize the benefits of AI research in healthcare, making them available across the globe.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/doctor-agreements.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lcc}
\hline
\textbf{Annotators} & \textbf{Kappa Score} & \textbf{Accuracy} \\ \hline
Doctor-1 vs. GPT-4            & 0.376                & 68.90\%                 \\
Doctor-2 vs. GPT-4            & 0.672                & 83.60\%                 \\
Doctor-1 vs. Doctor-2         & 0.416                & 70.80\%                 \\ \hline
\end{tabular}
\caption{Analysis of inter-annotator agreement between two medical doctors and GPT-4 on medical annotation validation.}
\label{tab: doctor-agreements}
\end{table*}

==> tables/dpo-experiments.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}          & \textbf{MedMCQA} & \textbf{MedQA} & \textbf{PubmedQA} & \textbf{USMLE-1} & \textbf{USMLE-2} & \textbf{USMLE-3} &\textbf{Avg.} \\ \midrule
medqa-Mistral           & 49.7             & 59.2           & 77.1              & 60.6             & 66.1             & 56.6             & 61.6         \\
medqa-pt-32-Mistral     & 51.5             & 60.9           & 76.5              & 55.3             & 65.1             & 57.4             & 61.1         \\ 

medqa-Mistral-dpo-1e-5   & 49.4             & 59.6          & 76.7              & 59.6             & 63.3             & 54.9             & 60.6          \\
medqa-Mistral-dpo-5e-5   & 49.2             & 59.4          & 76.7              & 58.5             & 61.5             & 52.5             & 59.6          \\          
medqa-Mistral-dpo-1e-4   & 49.3             & 57.3          & 77.3              & 56.4             & 62.4             & 54.9             & 59.6          \\
medqa-Mistral-dpo-b0.15  & 49.7             & 59.7          & 76.5              & 58.5             & 63.3             & 55.7             & 60.6          \\ 
medqa-Mistral-dpo-b0.2   & 49.7             & 59.8          & 76.7              & 57.5             & 64.2             & 54.9             & 60.5          \\ 
medqa-Mistral-dpo-b0.3   & 49.6             & 59.5          & 76.9              & 57.5             & 64.2             & 55.7             & 60.6          \\ 
medqa-Mistral-dpo-b0.5   & 49.6             & 59.6          & 77.0              & 57.5             & 64.2             & 55.7             & 60.6          \\ 
medqa-Mistral-dpo-kto    & 49.8             & 59.8          & 76.2              & 58.5             & 62.4             & 53.3             & 60.0          \\ 
medqa-Mistral-dpo-ipo    & 49.7             & 59.9          & 77.0              & 57.5             & 64.2             & 55.7             & 60.7          \\ 
medqa-Mistral-dpo-hinge  & 49.8             & 59.7          & 76.7              & 58.5             & 64.2             & 57.4             & 61.0          \\ 
medqa-Mistral-dpo-3e     & 49.1             & 60.1          & 76.3              & 58.5             & 63.3             & 54.1             & 60.2          \\ 
medqa-Mistral-dpo-ga8    & 49.4             & 59.5          & 76.5              & 57.5             & 64.2             & 54.9             & 60.3          \\ \bottomrule

\bottomrule
\end{tabular}
}
\caption{Zero-shot results on MedMCQA, PubMEDQA, MedQA, and USMLE by using the LM-Evaluation-Harness repository. USMLE scores are averaged among USMLE-step1, USMLE-step2, and USMLE-step3.}
\label{tab: dpo-zero-shot-acc}
\end{table*}

==> tables/few-shot-table.tex <==
\begin{table}[H]
\begin{center}
\begin{threeparttable}
\centering
\caption{Performance of different models on multiple choice components of MultiMedQA  \cite{singhal2022large}. {\DV} outperforms GPT-3.5 and Flan-PaLM 540B on every dataset except PubMedQA. {\DV} and GPT-3.5 were prompted with zero-shot direct prompts.}


    

\label{tab:multimedQA-scores} % table label for cross-referencing
\end{threeparttable} \\
\end{center}
\end{table}

==> tables/hippollama.tex <==
\begin{table*}[h!]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}                               & \textbf{MedMCQA}  & \textbf{MedQA}  & \textbf{PubmedQA}  & \textbf{USMLE-1}  & \textbf{USMLE-2}  & \textbf{USMLE-3}  &\textbf{Avg.}  \\ \midrule        
LLaMA2 7b                                    & 34.4              & 29.3            & 72.3               & 18.1              & 22.9              & 27.1              & 34.0          \\  
LLaMA2 7b + CP                               & 34.6              & 31.9            & 72.8               & 20.2              & 25.7              & 21.3              & 34.4          \\         
LLaMA2 7b + SFT                              & 52.7              & 49.7            & 75.7               & 37.2              & 42.2              & 44.3              & 50.3          \\ 
LLaMA2 7b + CP + SFT                         & 54.3              & 50.6            & 74.7               & 46.8              & 41.3              & 50.0              & 53.0          \\
LLaMA2 7b + CP + SFT + DPO                   & 54.4              & 50.4            & 74.8               & 46.8              & 39.5              & 49.2              & 52.5          \\
\bottomrule
\end{tabular}
}
\caption{\textbf{HippoLLaMA 7B: Analysis of Continued Pretraining, Instruction Tuning, and Direct Preference Optimization.} This table demonstrates the incremental impact of Continued Pretraining (CP) on medical text data, Instruction Tuning (SFT), and Direct Preference Optimization (DPO) on the zero-shot capabilities of the LLaMA2 7B model across a range of medical benchmarks, including MedMCQA, MedQA, PubmedQA, and the USMLE series. The results, aggregated and individual, underline the significance of each methodological advancement in enhancing the model's proficiency in interpreting and responding to complex medical queries, thereby providing a granular view of performance improvements at each stage of model optimization.}
\label{tab: hippollama}
\end{table*}

==> tables/llama-experiments-old.tex <==
\begin{table*}[h]
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccc}
\hline
\toprule
\textbf{Model}                      & \textbf{MedMCQA}  & \textbf{MedQA}  & \textbf{PubMedQA}  & \textbf{USMLE-1}  & \textbf{USMLE-2}  & \textbf{USMLE-3}  & \textbf{Avg.}   \\ \midrule
Llama2-7b                           & 34.4              & 29.3            & 72.3               & 18.1              & 22.9              & 27.1              & 34.0            \\ \midrule
Llama2-7b + PMC                     & 34.5              & 30.5            & 70.5               & 10.6              & 20.2              & 25.4              & 31.9            \\
Llama2-7b + GL                      & 34.8              & 32.3            & 71.1               & 20.2              & 22.0              & 26.2              & 34.4            \\
Llama2-7b + PMC + GL                & 34.9              & 32.0            & 69.4               & 17.0              & 22.9              & 27.9              & 34.0            \\ \midrule
Llama2-7b + SFT (6e-4)              & 32.4              & 30.4            & 66.7               & 19.2              & 22.9              & 24.6              & 32.7            \\
Llama2-7b + SFT (1e-4)              & 35.3              & 32.1            & 70.9               & 21.3              & 23.9              & 25.4              & 34.8            \\
Llama2-7b + SFT (6e-5)              & 35.2              & 34.7            & 71.5               & 23.4              & 29.4              & 23.8              & 36.3            \\
Llama2-7b + PMC + SFT               & 34.7              & 33.5            & 72.0               & 20.2              & 31.2              & 29.5              & 36.8            \\ 
Llama2-7b + GL  + SFT (6e-4)        & 32.4              & 32.9            & 61.6               & 21.3              & 23.9              & 22.1              & 32.4            \\
Llama2-7b + GL  + SFT (1e-4)        & 35.1              & 36.1            & 72.4               & 22.3              & 28.4              & 22.1              & 36.1            \\
Llama2-7b + GL  + SFT (6e-5)        & 34.8              & 34.0            & 72.9               & 23.4              & 23.9              & 26.2              & 35.9            \\
Llama2-7b + PMC + GL + SFT          & 34.7              & 32.4            & 71.2               & 23.4              & 26.6              & 24.6              & 35.5            \\ \midrule
Llama2-7b + SFT(a=8, r=8)           & 35.1              & 32.9            & 71.5               & 22.3              & 23.9              & 26.2              & 35.3            \\
Llama2-7b + SFT(a=16, r=16)         & 35.3              & 34.6            & 74.1               & 23.4              & 27.5              & 24.6              & 36.6            \\
Llama2-7b + SFT(a=32, r=32)         & 35.4              & 34.9            & 72.8               & 25.5              & 25.7              & 28.7              & 37.2            \\
Llama2-7b + SFT(a=64, r=64)         & 35.3              & 33.5            & 73.1               & 20.2              & 22.9              & 25.4              & 35.1            \\
Llama2-7b + SFT(a=128, r=128)       & 34.7              & 33.7            & 73.0               & 22.4              & 23.9              & 24.6              & 35.4            \\ \midrule
Llama2-7b + SFT(a=8, r=16)          & 35.3              & 32.1            & 70.9               & 21.3              & 23.9              & 25.4              & 34.8            \\
Llama2-7b + SFT(a=16, r=32)         & 34.7              & 34.1            & 72.9               & 21.3              & 24.8              & 25.4              & 35.5            \\
Llama2-7b + SFT(a=32, r=64)         & 34.8              & 34.9            & 72.9               & 28.7              & 26.6              & 29.5              & 37.9            \\
Llama2-7b + SFT(a=64, r=128)        & 35.4              & 34.2            & 73.2               & 21.3              & 27.5              & 23.0              & 35.8            \\
Llama2-7b + SFT(a=128, r=256)       & 34.1              & 32.5            & 72.9               & 23.4              & 28.4              & 27.9              & 36.5            \\ \midrule
Llama2-7b + SFT($FC$)               & 35.3              & 32.1            & 70.9               & 21.3              & 23.9              & 25.4              & 34.8            \\
Llama2-7b + SFT($Q,V$)              & 34.1              & 30.6            & 73.9               & 16.0              & 21.2              & 23.8              & 33.3            \\
Llama2-7b + SFT($FC,Q,V$)           & 35.2              & 35.3            & 71.9               & 18.1              & 30.3              & 28.7              & 36.6            \\ \midrule
Llama2-7b + GL + SFT(a=8, r=8)      & 36.3              & 35.0            & 70.4               & 19.2              & 27.5              & 28.7              & 36.2            \\
Llama2-7b + GL + SFT(a=16, r=16)    & 36.0              & 34.6            & 70.3               & 22.3              & 32.1              & 26.2              & 36.9            \\
Llama2-7b + GL + SFT(a=32, r=32)    & 37.7              & 36.3            & 71.4               & 28.7              & 32.1              & 30.3              & 39.4            \\
Llama2-7b + GL + SFT(a=64, r=64)    & 35.7              & 35.3            & 72.2               & 25.5              & 25.7              & 30.3              & 37.4            \\
Llama2-7b + GL + SFT(a=128, r=128)  & 34.9              & 34.2            & 70.2               & 22.3              & 23.9              & 30.3              & 36.0            \\ \midrule
Llama2-7b + GL + SFT(a=8, r=16)     & 35.1              & 36.1            & 72.4               & 22.3              & 28.4              & 22.1              & 36.1            \\
Llama2-7b + GL + SFT(a=16, r=32)    & 35.6              & 35.0            & 70.8               & 24.5              & 31.2              & 21.3              & 36.4            \\
Llama2-7b + GL + SFT(a=32, r=64)    & 35.7              & 36.1            & 72.6               & 27.7              & 27.5              & 28.7              & 38.0            \\
Llama2-7b + GL + SFT(a=64, r=128)   & 35.7              & 32.8            & 70.3               & 19.2              & 18.4              & 27.1              & 33.9            \\
Llama2-7b + GL + SFT(a=128, r=256)  & 33.7              & 33.2            & 69.6               & 21.3              & 29.4              & 26.2              & 35.6            \\ \midrule
Llama2-7b + GL + SFT($FC$)          & 35.1              & 36.1            & 72.4               & 22.3              & 28.4              & 22.1              & 36.1            \\
Llama2-7b + GL + SFT($Q,V$)         & 35.1              & 33.2            & 66.5               & 21.3              & 23.9              & 22.1              & 33.7            \\ 
Llama2-7b + GL + SFT($FC,Q,V$)      & 35.3              & 34.9            & 73.5               & 21.3              & 27.5              & 31.2              & 37.3            \\ \midrule

pub-Llama2-7b abs                   & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
medqa-Llama2-7b                     & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
medmc-Llama2-7b                     & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
evalo-all-Llama2-7b                 & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
evalo-abs-Llama2-7b                 & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
all-ra16-Llama2-7b                  & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
all-ra32-Llama2-7b                  & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
all-ra64-Llama2-7b                  & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\ \midrule
pt-32-Llama2-7b-evalo               & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
pt-32-Llama2-7b-medmc               & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
pt-32-Llama2-7b-medqa               & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
pt-32-Llama2-7b-pub                 & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
pt-32-Llama2-7b-all-ra16            & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
pt-32-Llama2-7b-all-ra32            & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\ \midrule

Llama2-7b + SFT + DPO               & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
Llama2-7b + SFT + KTO               & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
Llama2-7b + SFT + IPO               & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
Llama2-7b + SFT + Hinge             & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\ \midrule
Llama2-7b + PT + SFT + DPO          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
Llama2-7b + PT + SFT + KTO          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
Llama2-7b + PT + SFT + IPO          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\
Llama2-7b + PT + SFT + Hinge        & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO            \\ \bottomrule
\end{tabular}%  
}
\caption{llama TODOS}
\label{tab: llama-experiments}
\end{table*}


==> tables/main-results-few-shot.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}    & \textbf{MedMCQA} & \textbf{MedQA}  & \textbf{PubmedQA} & \textbf{USMLE-1} & \textbf{USMLE-2} & \textbf{USMLE-3} &\textbf{Avg.}        \\ 
                  & 5 Shot / 1 Shot  & 5 Shot / 1 Shot & 5 Shot / 1 Shot   & 5 Shot / 1 Shot  & 5 Shot / 1 Shot  & 5 Shot / 1 Shot  & 5 Shot / 1 Shot     \\ \toprule
LLaMA-2 7b        & 39.4 / TODO      & 39.5 / TODO     & 72.4 / TODO       & 22.3 / TODO      & 33.0 / TODO      & 32.0 / TODO      & TODO / TODO         \\
Mistral 7b        & 48.5 / TODO      & 48.9 / TODO     & 77.8 / TODO       & 50.0 / TODO      & 42.2 / TODO      & 43.4 / TODO      & TODO / TODO         \\  
BioMedLM          & 29.6 / TODO      & 30.6 / TODO     & 55.2 / TODO       & 22.3 / TODO      & 18.4 / TODO      & 31.2 / TODO      & TODO / TODO         \\
BioGPT-Large      & 33.1 / TODO      & 31.3 / TODO     & 60.1 / TODO       & 22.3 / TODO      & 22.0 / TODO      & 23.0 / TODO      & TODO / TODO         \\
Meditron 7b       & 38.2 / TODO      & 39.3 / TODO     & 75.7 / TODO       & 29.8 / TODO      & 30.3 / TODO      & 32.0 / TODO      & TODO / TODO         \\
Bio-Mistral 7b    & 42.4 / TODO      & 42.1 / TODO     & 75.1 / TODO       & 28.7 / TODO      & 34.9 / TODO      & 44.3 / TODO      & TODO / TODO         \\ \midrule
MedAlpaca 13b     & TODO / 32.0      & TODO / 33.0     & TODO / 74.2       & TODO / 21.3      & TODO / 25.7      & TODO / 32.0      & TODO / 36.4         \\  
PMC-LLaMA 13b     & TODO / 43.3      & TODO / 41.2     & TODO / 76.4       & TODO / 31.9      & TODO / 31.2      & TODO / 33.6      & TODO / 42.9         \\  
LLaMA-2 70b       & TODO / TODO      & TODO / TODO     & TODO / TODO       & TODO / TODO      & TODO / TODO      & TODO / TODO      & TODO / TODO         \\  
ClinicalCamel 70b & TODO / TODO      & TODO / TODO     & TODO / TODO       & TODO / TODO      & TODO / TODO      & TODO / TODO      & TODO / TODO         \\  
Meditron 70b      & TODO / TODO      & TODO / TODO     & TODO / TODO       & TODO / TODO      & TODO / TODO      & TODO / TODO      & TODO / TODO         \\ \midrule

HippoLLaMA 7b     & \textbf{53.9} / TODO  & 50.8 / TODO          & 76.6 / TODO           & 40.4 / TODO           & 39.5 / TODO          & 43.4 / TODO          & TODO / TODO  \\
HippoMistral 7b   & 51.8 / TODO           & \textbf{59.9} / TODO & \textbf{78.1} / TODO  & \textbf{61.7} / TODO  & \textbf{64.2} / TODO & \textbf{56.6} / TODO & TODO / TODO  \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Comparative analysis of generic and specialized medical LLMs across downstream medical tasks in few-shot learning settings.}
%Few-shot learning results} on MedMCQA, PubMEDQA, MedQA, and USMLE by using the LM-Evaluation-Harness repository. USMLE scores are averaged among USMLE-step1, USMLE-step2, and USMLE-step3.
}
\label{tab: main-results-few-shot}
\end{table*}

==> tables/main-results-zero-shot.tex <==
\begin{table}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}    & \textbf{MedMCQA} & \textbf{MedQA} & \textbf{PubmedQA} & \textbf{USMLE-1} & \textbf{USMLE-2} & \textbf{USMLE-3} &\textbf{Avg.} \\ \toprule
Gemma 2b          & 26.2             & 27.8           & 59.1              & 20.2             & 18.4             & 24.6             & 29.4         \\
LLaMA-2 7b        & 34.4             & 29.3           & 72.3              & 18.1             & 22.9             & 27.1             & 34.0         \\
Falcon 7b         & 30.5             & 27.9           & 65.3              & 18.1             & 26.6             & 23.8             & 32.0         \\
Vicuna 7b         & 35.9             & 35.1           & 70.9              & 25.5             & 27.5             & 33.6             & 38.1         \\
Mistral 7b        & 39.3             & 36.8           & 76.3              & 24.5             & 31.2             & 27.9             & 39.3         \\  
BioMedLM          & 32.2             & 29.3           & 55.2              & 15.9             & 19.3             & 23.0             & 25.9         \\
BioGPT-Large      & 33.1             & 31.3           & 60.1              & 22.3             & 22.0             & 23.0             & 32.0         \\
MedAlpaca 7b      & 35.8             & 36.1           & 73.2              & 22.3             & 27.5             & 29.5             & 37.4         \\
PMC-LLaMA 7b      & 31.5             & 28.0           & 66.5              & 21.3             & 23.9             & 22.1             & 32.2         \\
Meditron 7b       & 34.0             & 32.0           & 71.6              & 16.0             & 25.7             & 23.8             & 33.9         \\
Bio-Mistral 7b    & 36.4             & 35.0           & 73.4              & 24.5             & 27.5             & 27.9             & 37.5         \\ \midrule
LLaMA-2 13b       & 38.2             & 34.3           & 75.9              & 20.2             & 22.0             & 23.0             & 35.6         \\
Vicuna 13b        & 39.7             & 35.9           & 75.6              & 24.5             & 26.6             & 23.8             & 37.7         \\ 
MedAlpaca 13b     & 32.5             & 31.8           & 72.6              & 24.5             & 24.5             & 30.3             & 36.0         \\
PMC-LLaMA 13b     & 39.1             & 37.8           & 76.8              & 30.9             & 22.9             & 26.2             & 39.0         \\ 
ClinicalCamel 13b & 39.1             & 34.4           & 72.9              & 26.9             & 26.9             & 26.9             & 37.9         \\ \midrule
LLaMA-2 70b       & 42.8             & 44.9           & 73.2              & 31.9             & 44.0             & 44.3             & 46.8         \\
ClinicalCamel 70b & 43.7             & 45.5           & 73.6              & 40.4             & 43.1             & 42.6             & 48.2         \\
Meditron 70b      & 43.4             & 44.9           & 76.4              & 35.1             & 41.3             & 37.7             & 46.5         \\ \midrule
HippoLLaMA 7b     & \textbf{54.3}    & 50.6           & 74.7              & 46.8             & 41.3             & 50.0             & 53.0         \\
HippoMistral 7b   & 49.7             & \textbf{59.2}  & \textbf{77.1}     & \textbf{60.6}    & \textbf{66.1}    & \textbf{56.6}    & \textbf{61.6} \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Comparative analysis of generic and specialized medical LLMs across downstream medical tasks in zero-shot learning setting.}
%{Zero-shot results} on MedMCQA, PubMEDQA, MedQA, and USMLE by using the LM-Evaluation-Harness repository. USMLE scores are averaged among USMLE-step1, USMLE-step2, and USMLE-step3.
}
\label{tab: main-results-zero-shot}
\end{table}

==> tables/main_results-old.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{ 
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}    & \textbf{MedMCQA} & \textbf{MedQA} & \textbf{PubmedQA} & \textbf{USMLE-1} & \textbf{USMLE-2} & \textbf{USMLE-3} &\textbf{Avg.} \\ \midrule
LLaMA-2 7b        & 34.4             & 29.3           & 72.3              & 18.1             & 22.9             & 27.1             & 34.0         \\
Falcon 7b         & 30.5             & 27.9           & 65.3              & 18.1             & 26.6             & 23.8             & 32.0         \\
Vicuna 7b         & 35.9             & 35.1           & 70.9              & 25.5             & 27.5             & 33.6             & 38.1         \\
Mistral 7b        & 39.3             & 36.8           & 76.3              & 24.5             & 31.2             & 27.9             & 39.3         \\  
BioMedLM          & 32.2             & 29.3           & 55.2              & 15.9             & 19.3             & 23.0             & 25.9         \\
BioGPT-Large      & 33.1             & 31.3           & 60.1              & 22.3             & 22.0             & 23.0             & 32.0         \\
MedAlpaca 7b      & 35.8             & 36.1           & 73.2              & 22.3             & 27.5             & 29.5             & 37.4         \\
PMC-LLaMA 7b      & 31.5             & 28.0           & 66.5              & 21.3             & 23.9             & 22.1             & 32.2         \\
Meditron 7b       & 34.0             & 32.0           & 71.6              & 16.0             & 25.7             & 23.8             & 33.9         \\ \midrule
LLaMA-2 13b       & 38.2             & 34.3           & 75.9              & 20.2             & 22.0             & 23.0             & 35.6         \\
Vicuna 13b        & 39.7             & 35.9           & 75.6              & 24.5             & 26.6             & 23.8             & 37.7         \\ 
MedAlpaca 13b     & 32.5             & 31.8           & 72.6              & 24.5             & 24.5             & 30.3             & 36.0         \\
PMC-LLaMA 13b     & 39.1             & 37.8           & 76.8              & 30.9             & 22.9             & 26.2             & 39.0         \\ 
ClinicalCamel 13b & 39.1             & 34.4           & 72.9              & 26.9             & 26.9             & 26.9             & 37.9         \\ \midrule
LLaMA-2 70b       & 42.8             & 44.9           & 73.2              & 31.9             & 44.0             & 44.3             & 46.8         \\
ClinicalCamel 70b & 43.7             & 45.5           & 73.6              & 40.4             & 43.1             & 42.6             & 48.2         \\
Meditron 70b      & 43.4             & 44.9           & 76.4              & 35.1             & 41.3             & 37.7             & 46.5         \\ \midrule
HippoMistral 7b   & 49.7             & 59.2           & 77.1              & 60.6             & 66.1             & 56.6             & 61.6        \\ \bottomrule
\end{tabular}
}
\caption{Zero-shot results on MedMCQA, PubMEDQA, MedQA, and USMLE by using the LM-Evaluation-Harness repository. USMLE scores are averaged among USMLE-step1, USMLE-step2, and USMLE-step3.}
\label{tab: zero-shot-acc}
\end{table*}

==> tables/medmcqa_medqa_pubmedqa.tex <==
\definecolor{blue}{HTML}{008ED7}
\definecolor{mygray}{gray}{0.75}
\definecolor{lightBlue}{HTML}{e5f7ff}

\renewcommand{\familydefault}{\sfdefault}
\renewcommand{\arraystretch}{1.5}


\begin{center}
\begin{tabularx}{\textwidth}[t]{XX}
\arrayrulecolor{green}\hline
\textbf{\textcolor{myGreen}{Goal 1 Eradicate Extreme Poverty}} & \\
\hline
Target 1.A Halve, between 1990 and 2015, the proportion of the people whose income is less than \$1 a day. & 
\begin{minipage}[t]{\linewidth}%
\begin{itemize}
\item[1.1] Proportion of population below \$1 purchasing power parity (PPP) a day$^a$
\item[1.2] Poverty Gap ratio [incidence x depth of poverty]
\item[1.3] Share of the poorest quintile in national consumption
\end{itemize} 
\end{minipage}\\

\arrayrulecolor{black}\hline

Target 1.B Achieve full and productive employment and decent work for all, including women and young people &
\begin{minipage}[t]{\linewidth}%
\begin{itemize}
\item[1.4] Growth of GDP per person employed 
\item[1.5] Employment to population ratio
\item[1.6] Proportion of employed people living below \$1 (PP) a day
\item[1.7] Proportion of own-account and contribution family workers in total employment
\end{itemize} 
\end{minipage}\\

\hline

Target 1.C Halve, between 1990 and 2015, the proportion of people who suffer from hunger &
\begin{minipage}[t]{\linewidth}%
\begin{itemize}
\item[1.8] Prevalence of underweight children under five years of age
\item[1.9] Proportion of population below minimum level of dietary energy consumption
\end{itemize}
\end{minipage}\\

\arrayrulecolor{green}\hline
\textbf{\textcolor{myGreen}{Goal 2 Achieve universal primary education}} \\
\hline

Target 2.A Ensure that by 2015 children everywhere, boy and girls alike, will be able to complete a full course of primary schooling. &
\begin{minipage}[t]{\linewidth}%
\begin{itemize}
\item[2.1] Net enrollment ratio in primary education
\item[2.2] Proportion of pupils starting grade 1 who reach last grade of primary education
\item[2.3] Literacy rate of 15- to 24-year-olds, women and men
\end{itemize}
\end{minipage}\\

\hline
\multicolumn{2}{l}{%
\textbf{\textcolor{myGreen}{Goal 3 Promote gender equality and empower women}}} \\
\hline

Target 3.A Eliminate gender disparity in primary and secondary education, preferably by 2005, and in all levels of education no later than 2015 &
\begin{minipage}[t]{\linewidth}%
\begin{itemize}
\item[3.1] Ratios of girls to boys in primary, secondary and tertiary education
\item[3.2] Share of women in wage employment in the non-agricultural sector.
\end{itemize} 
\end{minipage}
\end{tabularx}
\end{center}



\begin{table*}[h]
\begin{tabular}{p{0.15\linewidth}p{0.85\linewidth}}
\toprule
\textbf{Task:}                      & MedMCQA               \\
\textbf{Documents:}                 & 4183                            \\
\multirow{2}{*}{\textbf{Question:}} & Tensor veli palatini is supplied by:                                                   \\
                                    & (A) Facial nerve (B) Trigeminal nerve (C) Glossopharyngeal nerve (D) Pharyngeal plexus \\
\textbf{Answer:}                    & \textless{}Output\textgreater{} \\ \bottomrule

\textbf{Task:}                      & MedQA                         \\
\textbf{Documents:}                 & 1273                            \\
\multirow{2}{*}{\textbf{Question:}} & A 3-week-old newborn is brought to the physician by his parents because of poor feeding, irritability, and frequent vomiting over the past week. The vomitus is greenish in color and smells strange. His parents have tried to feed him every 4 hours, but the patient often spits up or refuses to eat. The patient was born at term and had his first bowel movement at 50 hours of life. He has since had one bowel movement daily. He is at the 50th percentile for length, 10th percentile for weight, and 40th percentile for head circumference. He does not appear to be in acute distress. His temperature is 36.9°C (98.4°F), pulse is 140/min, respirations are 40/min, and blood pressure is 90/60 mm Hg. Physical examination shows that the patient has small, low-set ears, a broad and flat nasal bridge, and a large space between the first and second toes bilaterally. The abdomen is distended. When the finger is removed following a rectal exam, there is an explosive release of stool from the patient's rectum. An x-ray of the abdomen shows a section of dilated colon followed by a segment of colon without stool or air. Which of the following is most likely to confirm the diagnosis?                                                   \\
                                    & (A) CT scan of the abdomen (B) Transabdominal ultrasonography (C) Anorectal manometry (D) Rectal suction biopsy \\
\textbf{Answer:}                    & \textless{}Output\textgreater{} \\ \bottomrule

\textbf{Task:}                      & PubMedQA                         \\
\textbf{Documents:}                 & 1000                            \\
\textbf{Abstract:}                 &  The use of open access endoscopy is increasing. Its effect on the adequacy of patient informed consent, procedure acceptance and the impact on subsequent communication/transfer of procedure results to the patient have not been evaluated. The aim of our study was to compare the extent of preknowledge of procedures and test explanation, patient medical complexity, information transfer and overall patient satisfaction between a patient group referred for outpatient open access endoscopy versus a patient group from a gastrointestinal (GI) subspecialty clinic. Information was obtained from all patients presenting for outpatient upper and lower endoscopy by using a 1-page questionnaire. Patients from the two groups who had an outpatient upper/lower endoscopic procedure were contacted by phone after the procedure to obtain information with a standardized questionnaire. The open access patients reported receiving significantly less information to help them identify the procedure (p<0.01) and less explanation concerning the nature of the procedure than the group of patients referred from the subspecialty clinic (p<0.005). There was no difference between the two groups in satisfaction scores for examinations performed under conscious sedation. For flexible sigmoidoscopy without sedation, however, the GI clinic patient group were more satisfied with their procedure. The majority of patients, regardless of access, were more likely to receive endoscopic results from a gastroenterologist than the referring physician. Furthermore, the patients in the GI clinic group who underwent colonoscopy felt significantly better at follow-up. \\
\multirow{2}{*}{\textbf{Question:}} & Does open access endoscopy close the door to an adequately informed patient?                                                \\
                                    & (A) yes (B) no (C) maybe\\
\textbf{Answer:}                    & \textless{}Output\textgreater{} \\ \bottomrule


\end{tabular}%
\caption{Examples of prompts used in the evaluation of MedMCQA, MedQA, and PubMedQA, utilizing the LM-Evaluation-Harness Framework}
\label{tab: eval-medmcqa}
\end{table*}

==> tables/mistral-experiments-new.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}                            & \textbf{MedMCQA}  & \textbf{MedQA}  & \textbf{PubmedQA}  & \textbf{USMLE-1}  & \textbf{USMLE-2}  & \textbf{USMLE-3}  &\textbf{Avg.}  \\ \midrule           

Mistral 7B                                & 39.3              & 36.8            & 76.3                & 24.5             & 31.2              & 27.9              & 39.3          \\  \midrule

Mistral 7B + GL                            & 40.4              & 36.8            & 76.2               & 27.7              & 29.4              & 29.5              & 40.0          \\
Mistral 7B + GL (q,v)                      & 39.8              & 36.7            & 75.2               & 26.6              & 31.2              & 26.2              & 39.3          \\
Mistral 7B + GL (1e-4,32,32)               & 40.9              & 36.8            & 73.7               & 28.7              & 28.4              & 33.6              & 40.3          \\
Mistral 7B + GL (5e-5,32,32)               & 41.4              & 37.6            & 73.4               & 30.9              & 30.3              & 30.3              & 40.7          \\ % This
Mistral 7B + PMC                           & 39.4              & 36.4            & 75.9               & 27.6              & 30.3              & 29.5              & 39.9          \\
Mistral 7B + Pub                           & 38.0              & 35.7            & 77.1               & 24.5              & 27.5              & 31.2              & 39.0          \\
Mistral 7B + Pub + GL                      & 40.5              & 36.8            & 76.0               & 23.4              & 29.4              & 29.5              & 39.3          \\
Mistral 7B + PMC + GL + Pub                & 40.2              & 37.0            & 76.8               & 28.7              & 28.4              & 27.1              & 39.7          \\ \midrule  % This

%cutoff
Mistral 7B + GL                            & 41.4              & 38.4            & 74.8               & 28.7              & 31.2              & 31.2              & 40.9          \\
Mistral 7B + GL (5e-5,8,16)                & 41.4              & 36.5            & 75.3               & 28.7              & 31.2              & 26.2              & 39.9          \\
Mistral 7B + GL (1e-4,32,32)               & 40.9              & 37.2            & 74.2               & 27.7              & 29.4              & 31.2              & 40.1          \\
Mistral 7B + GL (5e-5,32,32)               & 41.6              & 38.0            & 73.7               & 31.9              & 31.2              & 30.3              & 41.1          \\
Mistral 7B + PMC                           & 40.0              & 37.9            & 75.2               & 25.5              & 30.3              & 33.6              & 40.4          \\
Mistral 7B + Pub                           & 39.0              & 36.2            & 78.2               & 26.6              & 27.5              & 32.0              & 39.9          \\
Mistral 7B + GL + PMC                      & 40.2              & 37.2            & 74.6               & 27.7              & 33.0              & 31.2              & 40.6          \\
Mistral 7B + GL + Pub                      & 41.0              & 37.9            & 76.8               & 24.5              & 34.9              & 31.2              & 41.0          \\ % This
Mistral 7B + GL + PMC + Pub                & 40.0              & 36.5            & 76.3               & 31.9              & 30.3              & 28.7              & 40.6          \\ \midrule

Mistral 7B + ood-it                         & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + pubqa                          & 23.3              & 24.5            & 76.6               & 20.2              & 19.3              & 29.5              & TODO          \\
Mistral 7B + medmcqa (32,32)                & 57.7              & 51.5            & 73.7               & 59.6              & 51.4              & 53.3              & 57.9          \\
Mistral 7B + medqa   (32,32)                & 50.0              & 59.4            & 78.9               & 54.3              & 59.6              & 59.8              & 60.3          \\
Mistral 7B + evals                          & 52.8              & 47.7            & 55.4               & 36.2              & 41.3              & 34.4              & TODO          \\
Mistral 7B + ood-it + evals                 & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\ \midrule 

Mistral 7B + (PMC + GL + Pub) + ood-it                         & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + (PMC + GL + Pub) + pubqa                          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + (PMC + GL + Pub) + medmcqa (32,32)                & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + (PMC + GL + Pub) + medqa   (32,32)                & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + (PMC + GL + Pub) + evals                          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + (PMC + GL + Pub) + ood-it + evals                 & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\ \midrule 

Mistral 7B + GL + ood-it                         & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + GL + pubqa                          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + GL + medmcqa (32,32)                & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + GL + medqa   (32,32)                & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + GL + evals                          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
Mistral 7B + GL + ood-it + evals                 & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\

\bottomrule
\end{tabular}
}
\caption{LLaMA2 7B Zero-shot results on MedMCQA, PubMEDQA, MedQA, and USMLE by using the LM-Evaluation-Harness repository. USMLE scores are averaged among USMLE-step1, USMLE-step2, and USMLE-step3.}
\label{tab: llama-zero-shot-acc}
\end{table*}

==> tables/mistral-experiments-old.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}    & \textbf{MedMCQA} & \textbf{MedQA} & \textbf{PubmedQA} & \textbf{USMLE-1} & \textbf{USMLE-2} & \textbf{USMLE-3} &\textbf{Avg.} \\ \toprule
Mistral 7b        & 39.3             & 36.8           & 76.3              & 24.5             & 31.2             & 27.9             & 39.3         \\  
Med-Mistral 7b    &\textbf{43.3}     &\textbf{44.5}   & 75.4              & \textbf{39.4}    &\textbf{37.6}     &\textbf{40.2}     &\textbf{46.7} \\ \midrule

Mistral-7b + PMC                            & 39.4              & 36.4            & 75.1               & 25.5              & 30.3              & 30.3              & 39.5            \\
Mistral-7b + PMC (bs8,ga2,r16,a16)          & 39.8              & 35.6            & 75.2               & 25.5              & 31.2              & 29.5              & 39.5            \\
Mistral-7b + GL (bs1,ga1,r8,a16)            & 38.2              & 35.6            & 75.1               & 28.7              & 26.6              & 29.5              & 38.9            \\
Mistral-7b + GL (bs8,ga2,r8,a16)            & 40.5              & 36.6            & 75.7               & 25.5              & 30.3              & 30.3              & 39.8            \\
Mistral-7b + GL (bs8,ga2,r16,a16)           & 41.5              & 36.8            & 73.8               & 30.9              & 36.7              & 32.0              & 41.9            \\
Mistral-7b + GL (bs8,ga2,r32,a32)           & 40.5              & 37.2            & 74.9               & 29.8              & 33.9              & 29.5              & 41.0            \\ %this
Mistral-7b + GL (bs16,ga2,r8,a16)           & 41.7              & 37.6            & 76.0               & 28.7              & 30.3              & 28.7              & 40.6            \\
Mistral-7b + GL (bs16,ga4,r8,a16)           & 41.2              & 37.6            & 75.9               & 24.5              & 31.2              & 28.7              & 39.9            \\
Mistral-7b + PMC + GL (bs8,ga2,r8,a16)      & 39.8              & 36.1            & 75.5               & 25.5              & 30.3              & 28.7              & 39.3            \\
Mistral-7b + PMC + GL (bs8,ga2,r16,a16)     & 39.8              & 36.9            & 75.3               & 29.8              & 26.6              & 27.1              & 39.2            \\
Mistral-7b + pub-all (bs8,ga2,r16,a16)      & 38.9              & 35.5            & 75.7               & 28.7              & 26.6              & 31.2              & 39.4            \\
Mistral-7b + pub-trn (bs8,ga2,r16,a16)      & 38.2              & 35.1            & 77.2               & 24.5              & 24.8              & 25.4              & 37.5            \\ \midrule

pub-Mistral               & 32.5             & 29.5           & 68.1              & 19.2             & 18.4             & 31.2             & 33.1         \\
pub-Mistral abs           & 32.5             & 29.5           & 60.4              & 19.2             & 18.4             & 31.2             & 31.9         \\
medqa-Mistral             & 49.7             & 59.2           & 77.1              & 60.6             & 66.1             & 56.6             & 61.6         \\ %this
medmc-Mistral             & 60.6             & 53.1           & 75.5              & 58.5             & 47.7             & 52.5             & 58.0         \\ 
evalo-all-Mistral         & 59.1             & 54.6           & 60.8              & 54.3             & 52.3             & 51.6             & 55.5         \\
evalo-abs-Mistral         & 59.1             & 54.6           & 72.7              & 54.3             & 52.3             & 51.6             & 57.4         \\ 
all-ra16-Mistral          & 51.2             & 53.0           & 76.8              & 47.9             & 47.7             & 45.1             & 53.6         \\ 
all-ra32-Mistral          & 51.2             & 48.9           & 75.6              & 52.1             & 37.6             & 47.5             & 52.1         \\ 
all-ra64-Mistral          & 46.9             & 43.5           & 73.2              & 39.4             & 32.1             & 45.1             & 46.7         \\ \midrule
pt-32-Mistral-evalo       & 58.1             & 54.8           & 73.6              & 53.2             & 56.0             & 50.0             & 57.6         \\
pt-32-Mistral-medmc       & 57.4             & 50.0           & 78.1              & 45.7             & 45.0             & 52.5             & 54.8         \\
pt-32-Mistral-medqa       & 51.5             & 60.9           & 76.5              & 55.3             & 65.1             & 57.4             & 61.1         \\ %this
pt-32-Mistral-pub         & 32.7             & 29.2           & 68.2              & 14.9             & 29.4             & 34.4             & 34.8         \\
pt-32-Mistral-all-ra16    & 53.7             & 53.9           & 76.5              & 48.9             & 50.5             & 57.4             & 56.8         \\ 
pt-32-Mistral-all-ra32    & 50.7             & 48.2           & 76.6              & 48.9             & 38.5             & 44.3             & 51.2         \\ \midrule

medqa-Mistral-dpo-1e-5   & 49.4             & 59.6          & 76.7              & 59.6             & 63.3             & 54.9             & 60.6          \\
medqa-Mistral-dpo-5e-5   & 49.2             & 59.4          & 76.7              & 58.5             & 61.5             & 52.5             & 59.6          \\          
medqa-Mistral-dpo-1e-4   & 49.3             & 57.3          & 77.3              & 56.4             & 62.4             & 54.9             & 59.6          \\ %this
medqa-Mistral-dpo-b0.15  & 49.7             & 59.7          & 76.5              & 58.5             & 63.3             & 55.7             & 60.6          \\ 
medqa-Mistral-dpo-b0.2   & 49.7             & 59.8          & 76.7              & 57.5             & 64.2             & 54.9             & 60.5          \\ 
medqa-Mistral-dpo-b0.3   & 49.6             & 59.5          & 76.9              & 57.5             & 64.2             & 55.7             & 60.6          \\ 
medqa-Mistral-dpo-b0.5   & 49.6             & 59.6          & 77.0              & 57.5             & 64.2             & 55.7             & 60.6          \\ 
medqa-Mistral-dpo-kto    & 49.8             & 59.8          & 76.2              & 58.5             & 62.4             & 53.3             & 60.0          \\ 
medqa-Mistral-dpo-ipo    & 49.7             & 59.9          & 77.0              & 57.5             & 64.2             & 55.7             & 60.7          \\ 
medqa-Mistral-dpo-hinge  & 49.8             & 59.7          & 76.7              & 58.5             & 64.2             & 57.4             & 61.0          \\ 
medqa-Mistral-dpo-3e     & 49.1             & 60.1          & 76.3              & 58.5             & 63.3             & 54.1             & 60.2          \\ 
medqa-Mistral-dpo-ga8    & 49.4             & 59.5          & 76.5              & 57.5             & 64.2             & 54.9             & 60.3          \\ \midrule

medmcqa-Mistral-dpo      & 60.4             & 52.6          & 74.9              & 57.5             & 45.0             & 54.1             & 57.4          \\
medmcqa-Mistral-kto      & 60.4             & 52.8          & 74.8              & 56.4             & 45.9             & 52.5             & 57.1          \\
medmcqa-Mistral-ipo      & 60.5             & 53.3          & 75.3              & 58.5             & 45.9             & 54.1             & 57.9          \\
medmcqa-Mistral-hinge    & 60.5             & 52.5          & 74.9              & 57.5             & 45.0             & 54.1             & 57.4          \\ 
evalall-Mistral-dpo      & 50.8             & 52.3          & 77.6              & 44.7             & 45.0             & 44.3             & 52.4          \\
evalall-Mistral-kto      & 50.7             & 52.0          & 77.5              & 46.8             & 45.0             & 48.4             & 53.4          \\
evalall-Mistral-ipo      & 51.1             & 52.6          & 76.8              & 46.8             & 48.6             & 45.9             & 53.6          \\
evalall-Mistral-hinge    & 50.8             & 52.2          & 77.0              & 46.8             & 45.0             & 45.1             & 52.8          \\ 
evalo-Mistral-dpo        & TODO             & TODO          & TODO              & TODO             & TODO             & TODO             & TODO          \\
evalo-Mistral-kto        & 58.8             & 54.8          & 72.6              & 55.3             & 48.6             & 50.8             & 56.8          \\
evalo-Mistral-ipo        & 59.0             & 54.7          & 72.9              & 54.2             & 51.4             & 50.8             & 57.2          \\
evalo-Mistral-hinge      & 58.9             & 54.7          & 72.9              & 54.2             & 53.2             & 50.8             & 57.4          \\ 
pubmed-Mistral-kto       & 33.0             & 28.9          & 68.7              & 21.3             & 20.2             & 30.3             & 33.7          \\
pubmed-Mistral-ipo       & 32.5             & 29.3          & 68.0              & 20.2             & 18.4             & 30.3             & 33.1          \\ \bottomrule

\bottomrule
\end{tabular}
}
\caption{Mistral 7B Zero-shot results on MedMCQA, PubMEDQA, MedQA, and USMLE by using the LM-Evaluation-Harness repository. USMLE scores are averaged among USMLE-step1, USMLE-step2, and USMLE-step3.}
\label{tab: mistral-zero-shot-acc}
\end{table*}

==> tables/mistral-experiments.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}                            & \textbf{MedMCQA}  & \textbf{MedQA}  & \textbf{PubmedQA}  & \textbf{USMLE-1}  & \textbf{USMLE-2}  & \textbf{USMLE-3}  &\textbf{Avg.}  \\ \midrule           
Mistral 7B                                & 39.3              & 36.8            & 76.3                & 24.5             & 31.2              & 27.9              & 39.3          \\  \midrule
$\;\;$ + Guidelines                            & 41.4              & 38.4            & 74.8               & 28.7              & 31.2              & 31.2              & 40.9          \\
$\;\;$ + PMC                           & 40.0              & 37.9            & 75.2               & 25.5              & 30.3              & 33.6              & 40.4          \\
$\;\;$ + Pub                           & 39.0              & 36.2            & 78.2               & 26.6              & 27.5              & 32.0              & 39.9          \\
$\;\;$ + Guidelines + PMC                      & 40.2              & 37.2            & 74.6               & 27.7              & 33.0              & 31.2              & 40.6          \\
$\;\;$ + Guidelines + PubMedQA                      & 41.0              & 37.9            & 76.8               & 24.5              & 34.9              & 31.2              & 41.0          \\ % This
$\;\;$ + Guidelines + PMC + PubMedQA                & 40.0              & 36.5            & 76.3               & 31.9              & 30.3              & 28.7              & 40.6          \\ \midrule
  
$\;\;$ + PubMedQA Instructions           & 32.5             & 29.5           & 60.4              & 19.2             & 18.4             & 31.2             & 31.9         \\
$\;\;$ + MedQA Instructions             & 49.7             & 59.2           & 77.1              & 60.6             & 66.1             & 56.6             & 61.6         \\ %this
$\;\;$ + MedMCQA Instructions             & 60.6             & 53.1           & 75.5              & 58.5             & 47.7             & 52.5             & 58.0         \\ 
$\;\;$ + General Instructions         & 59.1             & 54.6           & 60.8              & 54.3             & 52.3             & 51.6             & 55.5         \\
$\;\;$ + General Instructions + Evaluation Instructions          & 51.2             & 48.9           & 75.6              & 52.1             & 37.6             & 47.5             & 52.1         \\  \midrule

$\;\;$ + (PubMedQA + Guidelines) + General Instructions       & 58.1             & 54.8           & 73.6              & 53.2             & 56.0             & 50.0             & 57.6         \\
$\;\;$ + (PubMedQA + Guidelines) + MedMCQA Instructions       & 57.4             & 50.0           & 78.1              & 45.7             & 45.0             & 52.5             & 54.8         \\
$\;\;$ + (PubMedQA + Guidelines) + MedQA Instructions       & 51.5             & 60.9           & 76.5              & 55.3             & 65.1             & 57.4             & 61.1         \\ %this
$\;\;$ + (PubMedQA + Guidelines) + PubMedQA Instructions        & 32.7             & 29.2           & 68.2              & 14.9             & 29.4             & 34.4             & 34.8         \\
$\;\;$ + (PubMedQA + Guidelines) + General Instructions + Evaluation Instructions     & 50.7             & 48.2           & 76.6              & 48.9             & 38.5             & 44.3             & 51.2         \\ \midrule
         
$\;\;$ + (PubMedQA + Guidelines) + MedQA Instructions + DPO   & 49.3             & 57.3          & 77.3              & 56.4             & 62.4             & 54.9             & 59.6          \\  \bottomrule

\bottomrule
\end{tabular}
}
\caption{Mistral 7B Zero-shot experiments on MedMCQA, PubMEDQA, MedQA, and USMLE by using the LM-Evaluation-Harness repository. }
\label{tab: mistral-zero-shot-experiments}
\end{table*}

==> tables/overlap_sft.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lrccc}
\toprule
\textbf{Dataset}     & \textbf{Source}       & \textbf{MedMCQA (n=1,2,3)}       & \textbf{MedQA (n=1,2,3)}  & \textbf{PubmedQA(n=1,2,3)}     \\ \toprule
MedMCQA-train        & Meditron              & 5.76, 1.89, 0.6                  & 6.60, 2.58, 0.91          & 8.16, 2.30, 0.46               \\
MedQA-train          & Meditron              & 12.39, 2.95, 0.71                & 22.93, 10.62, 5.72        & 16.67, 4.41, 0.96              \\
PubMedQA-train       & Meditron              & 4.65, 0.85, 0.13                 & 4.74, 1.11, 0.22          & 7.77, 2.67, 0.70               \\
Ours        & Table 2                  & 2.29, 0.62, 0.13                 & 3.08, 1.25, 0.40          & 4.15, 1.25, 0.23               \\ \bottomrule
\end{tabular}%
}
\caption{Comparative analysis of n-gram percentage overlaps between Instruction-Tuning (IT) datasets and downstream evaluation test sets.}
\label{tab: sft-overlap}
\end{table}

==> tables/overlap_sft_numbers.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lrccc}
\toprule
\textbf{Dataset}     & \textbf{Source}       & \textbf{MedMCQA (n=1,2,3)}       & \textbf{MedQA (n=1,2,3)}    & \textbf{PubmedQA(n=1,2,3)}     \\ \toprule
MedMCQA-train        & Meditron              & 10269 - 20730 - 14242            & 11907 - 28874 - 21883       & 15723 - 27245 - 11453          \\
MedQA-train          & Meditron              & 7410 - 11024 - 5218              & 13251 - 39408 - 43039       & 12459 - 20032 - 8323           \\
PubMedQA-train       & Meditron              & 6990 - 8637 - 2746               & 7292 - 11595 - 4523         & 12784 - 29050 - 15318          \\
Ours                 & Table 2               & 9123 - 15237 - 7514              & 12260 - 31209 - 23395       & 16996 - 31802 - 13843          \\ \bottomrule
\end{tabular}%
}
\caption{Comparative analysis of n-gram percentage overlaps between Instruction-Tuning (IT) datasets and downstream evaluation test sets.}
\label{tab: sft-overlap-numbers}
\end{table}

==> tables/phi2-experiments.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}                        & \textbf{MedMCQA}  & \textbf{MedQA}  & \textbf{PubmedQA}  & \textbf{USMLE-1}  & \textbf{USMLE-2}  & \textbf{USMLE-3}  &\textbf{Avg.}  \\ \midrule           
phi-2                                 & 35.5              & 30.7            & 74.8               & 24.5              & 27.5              & 24.6              & TODO          \\  \midrule

phi-2 + GL                            & 33.4              & 30.2            & 62.5               & 27.7              & 25.7              & 24.6              & TODO          \\
phi-2 + GL  (5e-5,8,16)               & 33.5              & 29.5            & 64.6               & 22.3              & 25.7              & 26.2              & TODO          \\
phi-2 + GL (1e-4,16,16)               & 33.2              & 30.5            & 62.9               & 25.5              & 27.5              & 25.4              & TODO          \\
phi-2 + GL (1e-4,32,32)               & 33.3              & 30.7            & 61.0               & 20.2              & 24.8              & 25.4              & TODO          \\
phi-2 + PMC                           & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
phi-2 + PMC (6e-4,32,32)              & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
phi-2 + Pub                           & 33.3              & 31.5            & 65.5               & 27.7              & 27.5              & 29.5              & TODO          \\
phi-2 + Pub + GL                      & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
phi-2 + Pub + GL (6e-4)               & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
phi-2 + Pub + GL (q,v)                & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
phi-2 + PMC + GL                      & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\ 
phi-2 + PMC + GL + Pub                & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\ \midrule 

phi-2 + ood-it                         & 35.9              & 30.7            & 74.9               & 25.5              & 24.8              & 25.4              & TODO          \\
phi-2 + pubqa                          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
phi-2 + medmcqa                        & 44.0              & 35.9            & 58.2               & 36.2              & 30.3              & 30.3              & TODO          \\
phi-2 + medqa                          & 37.1              & 39.7            & 75.2               & 29.8              & 31.2              & 32.8              & TODO          \\
phi-2 + evals                          & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\
phi-2 + ood-it + evals                 & TODO              & TODO            & TODO               & TODO              & TODO              & TODO              & TODO          \\ \midrule

\bottomrule
\end{tabular}
}
\caption{phi-2 7B Zero-shot results on MedMCQA, PubMEDQA, MedQA, and USMLE by using the LM-Evaluation-Harness repository. USMLE scores are averaged among USMLE-step1, USMLE-step2, and USMLE-step3.}
\label{tab: phi-zero-shot-acc}
\end{table*}

==> tables/training-dataset.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l r r r r r}
\toprule
%\multicolumn{2}{c}{\textbf{Dataset}} & \textbf{Source} & \textbf{Size (MB)} & \textbf{\# of Samples} & \textbf{\# of Tokens} \\
\textbf{Task} & \textbf{Dataset} & \textbf{Source} & \textbf{Size (MB)} & \textbf{\# of Samples} & \textbf{\# of Tokens} & \textbf{License}\\
\midrule
\multirow{3}{*}{Pretraining Data} & Medical Guidelines & Meditron & 382.6 & 37,970 & 96,106,387 & Apache 2.0 License  \\
& PMC-Patients & Pubmed Central & 462.3 & 167,034 & 122,237,987 & CC BY-NC-SA 4.0 \\
& PubMedQA-train & PubMedQA & 290.2 & 211,269 & 80,353,116 & MIT License \\
\midrule
%\multicolumn{2}{l}{Final Dataset} & Ours & 1135.1 & 416,273 & TODO \\
%\midrule
\multirow{9}{*}{OOD IT Data} & Medical Flashcards & MedAlpaca & 18.8 & 33,955 & 3,848,490  & CC BY 4.0 \\
& GenMedGPT-5k & ChatDoctor & 3.1 & 5,452 & 604,258 & CC BY 4.0 \\
& Open-Platypus & Platypus & 32.9 & 24,926 & 9,494,869 & CC BY 4.0 \\
& HealthCareMagic-100k & ChatDoctor & 143.8 & 112,165 & 32,280,631 & CC BY 4.0 \\
& UMLS & PMC-LLaMA & 23.0 & 49,057 & 4,638,385 & CC BY 4.0 \\
& UMLS-Relations & PMC-LLaMA & 21.7 & 50,000 & 4,316,274 & CC BY 4.0 \\
& WikiDoc & MedAlpaca & 11.0 & 10,000 & 2,637,965 & CC BY 4.0 \\
& WikiDoc-Patient-Info & MedAlpaca & 3.7 & 5,942 & 779,319 & CC BY 4.0 \\
& MedicationQA & PMC-LLaMA & 0.4 & 552 & 78,132 & CC BY 4.0 \\
\midrule
%\multicolumn{2}{l}{Final Dataset} & Ours & 258.4 & 292,049 & TODO \\
%\midrule
\multirow{3}{*}{Evaluation IT Data} & MedMCQA-train & MedMCQA & 114.4 & 182,822 & 24,868,082 & CC BY 4.0 \\
& MedQA-train & MedQA & 14.2 & 10,178 & 3,384,646 & CC BY 4.0 \\
& PubMedQA-train & PubMedQA & 76.3 & 211,269 & 95,850,875 & CC BY 4.0 \\
\midrule
%\multicolumn{2}{l}{Final Dataset} & Ours & 204.9 & 403,269 & TODO \\
Preference Data & Medical Comparisons & iCliniq & 28.7 & 15,258 & 6,322,344 & CC BY 4.0 \\
\midrule
\multirow{6}{*}{Downstream Test Data} 
& MedMCQA-test  & MedMCQA  & 1.6 & 4,183 & 252,763 & CC BY 4.0 \\
& MedQA-test    & MedQA    & 1.0  & 1,273  & 311,539 & CC BY 4.0 \\
& PubMedQA-test & PubMedQA & 1.1  & 1000   & 387,649 & CC BY 4.0 \\
& USMLE-step1   & USMLE    & 0.1  & 94     & 21,432 & CC BY 4.0 \\
& USMLE-step2   & USMLE    & 0.1  & 109    & 36,020 & CC BY 4.0 \\
& USMLE-step3   & USMLE    & 0.1  & 122    & 42,240 & CC BY 4.0 \\
\bottomrule
\end{tabular}%
}
\caption{Proposed continued training dataset.}
\label{tab: all-data}
\end{table}


==> tables/usmle.tex <==
\begin{table*}[h]
\begin{tabular}{p{0.15\linewidth}p{0.85\linewidth}}
\toprule
\textbf{Task:}                      & USMLE-Step1               \\
\textbf{Documents:}                 & 94                            \\
\multirow{2}{*}{\textbf{Question:}} & A 58-year-old man with chronic obstructive pulmonary disease comes to the clinic with his wife for a follow-up examination. He has smoked one pack of cigarettes daily for 35 years. He has tried to quit smoking twice but was unsuccessful both times. At today’s visit, when the physician asks the patient about smoking cessation, he says he is not ready to do so. The patient’s wife states her husband’s smoking makes her cough and gives her chest tightness. Which of the following is the most appropriate physician statement?                                                   \\
                                    & (A) "Are there any reasons why you might want to quit smoking?" (B) "Are you aware that your lung condition is chronic at this point?" (C) "I'm sure you don't want your wife to suffer as a result of your smoking." (D) "The majority of your health issues would improve if you quit smoking." (E) "Why haven't you been able to stay off cigarettes?" \\
\textbf{Answer:}                    & \textless{}Output\textgreater{} \\ \bottomrule

\textbf{Task:}                      & USMLE-Step2                          \\
\textbf{Documents:}                 & 109                            \\
\multirow{2}{*}{\textbf{Question:}} & A 32-year-old woman comes to the emergency department because of a 1-day history of sharp, right-sided chest pain that worsens with coughing and sneezing. Four days ago, she had a mild sore throat and runny nose followed by nonproductive cough 1 day later. Over-the-counter decongestant and aspirin mildly relieved the symptoms. She has not had shortness of breath, blood-tinged sputum, fever, or chills. She has a long-standing history of recurrent aphthous ulcers. Her only medication is an oral contraceptive. Temperature is 37.2°C (99.0°F), pulse is 65/min, and respirations are 14/min. Pulse oximetry on room air shows an oxygen saturation of 99\%. Splinting is observed over the right hemithorax with deep breathing. On cardiac examination, no abnormalities are heard. The remainder of the examination shows no abnormalities. Chest x-ray shows no abnormalities. Which of the following is the most appropriate next step in management?    \\
                                    & (A) Azithromycin therapy (B) CT angiography (C) Electrocardiography (D) Ibuprofen therapy (E) Prednisone therapy (F) Transthoracic echocardiography  \\
\textbf{Answer:}                    & \textless{}Output\textgreater{} \\ \bottomrule

\textbf{Task:}                      & USMLE-Step3                          \\
\textbf{Documents:}                 & 122                            \\
\multirow{2}{*}{\textbf{Question:}} & A 57-year-old woman comes to the office for a preoperative evaluation 2 weeks before undergoing scheduled laparoscopic cholecystectomy. Medical history is otherwise unremarkable and the patient takes no medications. Family history is significant for stable angina in her father and rheumatoid arthritis in her mother. The patient has a 102-year-old grandmother who resides in a nursing care facility and has Parkinson disease. The patient does not smoke cigarettes or drink alcoholic beverages. During the interview, her face is expressionless. She has a flexed posture and is unable to open her mouth wide. She is 173 cm (5 ft 8 in) tall and weighs 81 kg (179 lb); BMI is 27 kg/m2. Vital signs are normal. Physical examination discloses thickening and hardening of the skin over the dorsum of the hands and forearms, as well as mild kyphosis. Strength testing shows no abnormalities; muscle tension is normal. Passive and active range of motion of the upper extremities is full. Gait is slow and deliberate. The remainder of the physical examination discloses no abnormalities. Prior to surgery, further evaluation is indicated for which of the following conditions in this patient?       \\
                                    & (A) Osteitis deformans (Paget disease) (B) Parkinson disease (C) Progressive supranuclear palsy (D) Sarcopenia (E) Systemic sclerosis (scleroderma) \\
\textbf{Answer:}                    & \textless{}Output\textgreater{} \\ \bottomrule


\end{tabular}%
\caption{Examples of prompts used in the evaluation of USMLE-Step1, USMLE-Step2, and USMLE-Step3, utilizing the LM-Evaluation-Harness Framework.}
\label{tab: eval-usmle}
\end{table*}
